Unscrambling the Rectification of Adversarial Attacks Transferability across Computer Networks

Convolutional neural networks (CNNs) models play a vital role in achieving state-of-the-art performances in various technological fields. CNNs are not limited to Natural Language Processing (NLP) or Computer Vision (CV) but also have substantial applications in other technological domains, particularly in cybersecurity. The reliability of CNN's models can be compromised because of their susceptibility to adversarial attacks, which can be generated effortlessly, easily applied, and transferred in real-world scenarios. In this paper, we present a novel and comprehensive method to improve the strength of attacks and assess the transferability of adversarial examples in CNNs when such strength changes, as well as whether the transferability property issue exists in computer network applications. In the context of our study, we initially examined six distinct modes of attack: the Carlini and Wagner (C&W), Fast Gradient Sign Method (FGSM), Iterative Fast Gradient Sign Method (I-FGSM), Jacobian-based Saliency Map (JSMA), Limited-memory Broyden fletcher Goldfarb Shanno (L-BFGS), and Projected Gradient Descent (PGD) attack. We applied these attack techniques on two popular datasets: the CIC and UNSW datasets. The outcomes of our experiment demonstrate that an improvement in transferability occurs in the targeted scenarios for FGSM, JSMA, LBFGS, and other attacks. Our findings further indicate that the threats to security posed by adversarial examples, even in computer network applications, necessitate the development of novel defense mechanisms to enhance the security of DL-based techniques.

==> IEEE_TNSM_Template.tex <==
% The paper headers
\markboth{Journal of \LaTeX\ Class Files,~Vol.~14, No.~8, August~2015}%
{Shell \MakeLowercase{\textit{et al.}}: Bare Demo of IEEEtran.cls for IEEE Communications Society Journals}

\appendices
\section{Proof of the First Zonklar Equation}
Appendix one text goes here.

% you can choose not to have a title for an appendix
% if you want by leaving the argument blank
\section{}
Appendix two text goes here.


% use section* for acknowledgment
\section*{Acknowledgment}


The authors would like to thank...


% Can use something like this to put references on a page
% by themselves when using endfloat and the captionsoff option.
\ifCLASSOPTIONcaptionsoff
  \newpage
\fi



% trigger a \newpage just before the given reference
% number - used to balance the columns on the last page
% adjust value as needed - may need to be readjusted if
% the document is modified later
%\IEEEtriggeratref{8}
% The "triggered" command can be changed if desired:
%\IEEEtriggercmd{\enlargethispage{-5in}}

% references section

% can use a bibliography generated by BibTeX as a .bbl file
% BibTeX documentation can be easily obtained at:
% http://mirror.ctan.org/biblio/bibtex/contrib/doc/
% The IEEEtran BibTeX style support page is at:
% http://www.michaelshell.org/tex/ieeetran/bibtex/
%\bibliographystyle{IEEEtran}
% argument is your BibTeX string definitions and bibliography database(s)
%\bibliography{IEEEabrv,../bib/paper}
%
% <OR> manually copy in the resultant .bbl file
% set second argument of \begin to the number of references
% (used to reserve space for the reference number labels box)
\begin{thebibliography}{1}

\bibitem{IEEEhowto:kopka}
H.~Kopka and P.~W. Daly, \emph{A Guide to \LaTeX}, 3rd~ed.\hskip 1em plus
  0.5em minus 0.4em\relax Harlow, England: Addison-Wesley, 1999.

\end{thebibliography}

% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

\begin{IEEEbiography}{Michael Shell}
Biography text here.
\end{IEEEbiography}

% if you will not have a photo at all:
\begin{IEEEbiographynophoto}{John Doe}
Biography text here.
\end{IEEEbiographynophoto}

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage

\begin{IEEEbiographynophoto}{Jane Doe}
Biography text here.
\end{IEEEbiographynophoto}

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}



% that's all folks

==> Tables/Abbreviations.tex <==
\begin{table}[!t]
%\scriptsize
%\footnotesize
\centering
\caption{Abbreviation and Notation List. \label{Abbreviations}}
\begin{tabular}{@{}|c|l|}
\hline
\textbf{Acronym} & \textbf{Description} \\ \hline

CNN & Convolutional Neural Network \\ \hline

%LSTM & \red{Long Short-Term Memory Networks} \\ \hline

%\red{SN} & \red{Source Network} \\ \hline

%\red{TN} & \red{Target Network} \\ \hline

LK & Limited Knowledge \\ \hline

PK & Perfect Knowledge \\ \hline

CF & Counter Forensics \\ \hline

DL, ML & Deep Learning, Machine Learning \\ \hline

%ML & Machine Learning \\ \hline

SN, TN & Source Network, Target Network \\ \hline

%TN & Target Network \\ \hline

CM  & Cross Model \\ \hline

CT  & Cross Training\\ \hline

CMT  & Cross Model and Training\\ \hline

ASR & Average Attack Success Rate \\ \hline

Max. dist & Average Maximum distortion\\ \hline

PSNR & Average Peak signal-to-noise ratio\\ \hline

$L_1$ dist & Average $L_1$ distance\\ \hline

FGSM & Fast Gradient Sign Method\\ \hline


I-FGSM & Iterative Fast Gradient Sign Method \\ \hline

JSMA  & Jacobian-based Saliency Map Attack\\ \hline

LBFGS  & Limited-memory Broyden-Fletcher-Goldfarb-Shanno\\ \hline
C\&W & Carlini and Wagner \\ \hline
PGD  & Projected Gradient Descent\\ \hline

CIC  & Canadian Institute for Cybersecurity\\ \hline

DGA  & Domain Generating algorithms\\ \hline

DN  & Domain Name\\ \hline

RNN & Recurrent Neural Network\\ \hline

DDoS  & Distributed Denial of Service\\ \hline

%$\varepsilon$ & Normalized Attack Strength Factor\\ \hline

%$\theta$ & Model parameters\\ \hline

\end{tabular}
\end{table}

==> Tables/Cases.tex <==
\begin{table}[!h]

%\scriptsize
\centering
\caption{Scenarios of the Considered Source and Target Networks.\label{Cases}}
\begin{threeparttable}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\backslashbox{\textbf{SN}}{\textbf{TN}} & \bm{$N_{1}$}  & \bm{$N_{2}$} & \bm{$N_{3}$} & \bm{$N_{4}$} & \bm{$N_{5}$} & \bm{$N_{6}$} \\ \hline

\bm{$N_{1}$} & \cellcolor{grey} & CT &  CM &   CMT & CT& \cellcolor{grey} \TBstrut\\\hline

\bm{$N_{2}$} &  CT &  \cellcolor{grey}& \cellcolor{grey} &   CM &\cellcolor{grey}&\cellcolor{grey}\TBstrut\\\hline

\bm{$N_{3}$} &  CM  & \cellcolor{grey} & \cellcolor{grey} &   CT &\cellcolor{grey}&\cellcolor{grey} \TBstrut\\\hline

\bm{$N_{4}$ }&  CMT  &  CM  &  CT & \cellcolor{grey} &\cellcolor{grey}&\cellcolor{grey}\TBstrut\\\hline

\bm{$N_{5}$} & \cellcolor{grey} &  \cellcolor{grey}  & \cellcolor{grey} & \cellcolor{grey} &\cellcolor{grey}&CM\TBstrut\\\hline

\bm{$N_{6}$} & \cellcolor{grey}  &  \cellcolor{grey}  & \cellcolor{grey} & \cellcolor{grey} &\cellcolor{grey}&CMT\TBstrut\\\hline


\end{tabular}

\begin{tablenotes}
      \small
      \item \small
    \bm{$N_{1}$}:$N_{SPRITZ1}^{N-BaIoT}$, \bm{$N_{2}$}:$N_{SPRITZ1}^{DGA}$, \bm{$N_{3}$}:$N_{SPRITZ2}^{N-BaIoT}$,  
\end{tablenotes}

\begin{tablenotes}
      \small
      \item \small \bm{$N_{4}$}:$N_{SPRITZ2}^{DGA}$ \bm{$N_{5}$}:$N_{SPRITZ1}^{RIPE}$,  \bm{$N_{6}$}:$N_{SPRITZ2}^{N-RIPE}$
    
\end{tablenotes}
\end{threeparttable}
%\begin{tablenotes}
 %     \small
  %  $N_{1}$:$N_{SPRITZ1}^{N-BaIoT}$, %$N_{2}$:$N_{SPRITZ1}^{DGA}$, $N_{3}$:$N_{SPRITZ2}^{N-BaIoT}$, %$N_{4}$:$N_{SPRITZ2}^{DGA}$, $N_{5}$:$N_{SPRITZ1}^{RIPE}$,  %$N_{6}$:$N_{SPRITZ2}^{N-RIPE}$
   % \end{tablenotes}

\end{table}


==> Tables/CrossTraining/CT_SPRITZ1_First.tex <==
\newpage
\begin{table*}[!h]
%\scriptsize
\centering
\caption{Experimental results for Cross Model and Training Transferability\\. \label{CMT}}
\resizebox{2\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{SN} & \textbf{TN} & \textbf{Accuracy} & \textbf{Attack Type} & \textbf{PSNR} & \textbf{$L_1$ dist} & \textbf{Max. dist} & \textbf{ASR} & \textbf{ASR} \TBstrut\\
& & & & & & & \textbf{(SN)} & \textbf{(TN)}  \\ \hline
 \rowcolor{grey}
$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{DGA}$ & SN = 98.80\% , TN = 100\% & I-FGSM, $\varepsilon$ = 0.1 & 18.65 & 22.07 & 64.78  & 1.0000 & 0.0030 \TBstrut\\ \hline

$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{DGA}$ & SN = 98.80\% , TN = 100\% & I-FGSM, $\varepsilon$ = 0.01 & 18.93 & 21.26 & 62.71  & 1.0000 & 0.0000 \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{DGA}$ & SN = 98.80\% , TN = 100\% & I-FGSM, $\varepsilon$ = 0.001 & 19.06 & 20.93 & 61.72  & 1.0000 & 0.0000 \TBstrut\\ \hline

$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{DGA}$ & SN = 98.80\% , TN = 100\% & JSMA, $\theta$ = 0.1 & 18.49 & 7.29  & 178.50 & 1.0000 & 0.0000 \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{DGA}$ & SN = 98.80\% , TN = 100\% & JSMA, $\theta$ = 0.01 & --     & --     & --      & FAIL\textsuperscript{*}   & --      \TBstrut\\ \hline

$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{DGA}$ & SN = 98.80\% , TN = 100\% & LBFGS, default parameter & 22.57 & 10.46 & 110.67 & 0.9910 & 0.0000 \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{DGA}$ & SN = 98.80\% , TN = 100\% & PGD, default parameter & 19.59 & 19.71 & 54.00  & 1.0000 & 0.0000 \TBstrut\\ \hline

$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{DGA}$ & SN = 98.80\% , TN = 100\% & DeepFool, default parameter & 20.87 & 12.14 & 143.19 & 0.9676 & 0.0324 \TBstrut\\ \hline

 \rowcolor{grey}
$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{N-BaIoT}$ & SN = 99.60\% , TN = 99.60\% & I-FGSM, $\varepsilon$ = 0.1 & 28.49 & 6.03 & 24.15 & 1.0000 & 0.0400 \TBstrut\\ \hline

$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{N-BaIoT}$ & SN = 99.60\% , TN = 99.60\% & I-FGSM, $\varepsilon$ = 0.01 & 28.62 & 5.99 & 23.25 & 1.0000 & 0.0000 \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{N-BaIoT}$ & SN = 99.60\% , TN = 99.60\% & I-FGSM, $\varepsilon$ = 0.001 & 28.92 & 5.76 & 22.64 & 1.0000 & 0.0000 \TBstrut\\ \hline

$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{N-BaIoT}$ & SN = 99.60\% , TN = 99.60\% & JSMA, $\theta$ = 0.1 & 31.17 & 1.28 & 56.56 & 1.0000 & 0.0000  \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{N-BaIoT}$ & SN = 99.60\% , TN = 99.60\% & JSMA, $\theta$ = 0.01 & --     & --    & --     & FAIL\textsuperscript{*}   & --      \TBstrut\\ \hline

$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{N-BaIoT}$ & SN = 99.60\% , TN = 99.60\% & LBFGS, default parameter & 34.22 & 1.40 & 33.93 & 0.9860 & 0.0040 \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{N-BaIoT}$ & SN = 99.60\% , TN = 99.60\% & PGD, default parameter & 29.24 & 5.99 & 22.24 & 1.0000 & 0.0000 \TBstrut\\ \hline

$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{N-BaIoT}$ & SN = 99.60\% , TN = 99.60\% & DeepFool, default parameter & 31.02 & 2.59 & 53.42 & 1.0000 & 0.0104 \TBstrut\\ \hline

 \rowcolor{grey}
$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{RIPE}$ & SN = 98.80\% , TN = 99.80\% & I-FGSM, $\varepsilon$ = 0.1 & 18.65 & 22.07 & 64.78  & 1.0000 & 0.0000 \TBstrut\\ \hline

$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{RIPE}$ & SN = 98.80\% , TN = 99.80\% & JSMA, $\theta$ = 0.1 & 18.49 & 7.29  & 178.50 & 1.0000 & 0.0010 \TBstrut\\ \hline

 \rowcolor{grey}
$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{RIPE}$ & SN = 98.80\% , TN = 99.80\% & LBFGS, default parameter & 22.57 & 10.46 & 110.67 & 0.9910 & 0.0000 \TBstrut\\ \hline


$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{RIPE}$ & SN = 98.80\% , TN = 99.80\% & PGD, default parameter & 19.59 & 19.71 & 54.00  & 1.0000 & 0.0000 \TBstrut\\ \hline

\rowcolor{grey}
$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{RIPE}$ & SN = 98.80\% , TN = 99.80\% & DeepFool, default parameter & 20.87 & 12.14 & 143.19 & 0.9676 & 0.0200 \TBstrut\\ \hline

\end{tabular}}
\\FAIL\textsuperscript{*}: In this case, the attack on the source network fails and we cannot transfer it to the target network. Therefore, the numerical values of the average PSNR, the average $L_1$ dist, and the average maximum distortion are not possible. 
\end{table*}












==> Tables/CrossTraining/deniz_cross_training.tex <==

\newpage
\begin{table}[ht!]
\centering
\paperwidth
\resizebox{2\columnwidth}{!}{\begin{tabular}{|c|c|c|c|c|c|c|c|}
 \hline
 \textbf{SN} & \textbf{TN} & \textbf{Attack Type} & \textbf{PSNR} & \textbf{\(L_1\) Dist} & \textbf{Max Distance} & \textbf{ASR (SN)} & \textbf{ASR (TN)} \\ 
 \hline
$N_{QUB1}^{UNSW}$ & $N_{QUB1}^{CIC}$  & I-FGSM (\epsilon=0.1) & 41.11 & 2.00 & 2.55 & 1.00 & 0.90\\
 \hline
$N_{QUB1}^{UNSW}$ & $N_{QUB1}^{CIC}$  & I-FGSM (\epsilon=0.01) & 40.27 & 2.04 & 3.56 & 1.00 & 0.31\\ 
 \hline
$N_{QUB1}^{UNSW}$ & $N_{QUB1}^{CIC}$   & I-FGSM (\epsilon=0.001) &40.08 &2.08 &3.69 &1.00 &0.21 \\
 \hline
$N_{QUB1}^{UNSW}$ & $N_{QUB1}^{CIC}$  & FGSM (\epsilon=0.1) &41.11 &2.00 &2.55 &1.00 &0.90 \\
 \hline
$N_{QUB1}^{UNSW}$ & $N_{QUB1}^{CIC}$ & FGSM (\epsilon=0.01) &40.71 &2.10 &2.66 &1.00 &0.82 \\
 \hline
$N_{QUB1}^{UNSW}$ & $N_{QUB1}^{CIC}$  & FGSM (\epsilon=0.001) &41.07 &2.04 &2.57 &1.00 &0.81 \\
 \hline
$N_{QUB1}^{UNSW}$ & $N_{QUB1}^{CIC}$   & JSMA (\theta=0.1) &41.06 &0.07 &93.47 &1.00 &0.83 \\
 \hline
$N_{QUB1}^{UNSW}$ & $N_{QUB1}^{CIC}$  & JSMA (\theta=0.01) &44.07 &0.16 &17.85 &1.00 &0.13 \\
 \hline
$N_{QUB1}^{UNSW}$ & $N_{QUB1}^{CIC}$   & LBFGS (\textit{default parameter})&15.48&31.52&205.10&1.00&0.71 \\
 \hline
$N_{QUB1}^{UNSW}$ & $N_{QUB1}^{CIC}$  & PGD (\textit{default parameter})&40.90 &1.90 &3.32 &1.00 &0.15 \\
 \hline
$N_{QUB1}^{UNSW}$ & $N_{QUB1}^{CIC}$ & DeepFool (\textit{default parameter}) &-&-&-&FAIL &- \\
 \hline
$N_{QUB1}^{UNSW}$ & $N_{QUB1}^{CIC}$ & CW (\textit{default parameter}) &-&-&-&- &- \\
 \hline




$N_{QUB1}^{CIC}$ & $N_{QUB1}^{UNSW}$  & I-FGSM (\epsilon=0.1) & 41.94 & 1.65 & 2.55 & 1.00 & 0.97\\
\hline
$N_{QUB1}^{CIC}$ & $N_{QUB1}^{UNSW}$  & I-FGSM (\epsilon=0.01) & 40.51 &1.88 & 3.59 & 1.00 & 0.73\\ 
\hline
$N_{QUB1}^{CIC}$ & $N_{QUB1}^{UNSW}$  & I-FGSM (\epsilon=0.001) &40.03 &1.97 &3.83 &1.00 &0.73 \\
\hline
$N_{QUB1}^{CIC}$ & $N_{QUB1}^{UNSW}$   & FGSM (\epsilon=0.1) &44.90 &1.20 &1.91 &1.00 &0.97 \\
\hline
$N_{QUB1}^{CIC}$ & $N_{QUB1}^{UNSW}$  & FGSM (\epsilon=0.01) &41.94 &1.65 &2.55 &1.00 &0.97 \\
\hline
$N_{QUB1}^{CIC}$ & $N_{QUB1}^{UNSW}$   & FGSM (\epsilon=0.001) &49.79 &0.78 &1.27 &1.00 &0.97 \\
\hline
$N_{QUB1}^{CIC}$ & $N_{QUB1}^{UNSW}$   & JSMA (\theta=0.1) &50.88 &0.03 &25.49 &1.00 &0.98 \\
\hline
$N_{QUB1}^{CIC}$ & $N_{QUB1}^{UNSW}$   & JSMA (\theta=0.01) &53.59 &0.03 &13.00 &1.00 &0.98 \\
\hline
$N_{QUB1}^{CIC}$ & $N_{QUB1}^{UNSW}$  & LBFGS (\textit{default parameter})&21.20&12.27&195.85&1.00&0.42 \\
\hline
$N_{QUB1}^{CIC}$ & $N_{QUB1}^{UNSW}$  & PGD (\textit{default parameter})&41.49 &1.69 &3.12 &1.00 &0.73 \\
\hline
$N_{QUB1}^{CIC}$ & $N_{QUB1}^{UNSW}$  & DeepFool (\textit{default parameter}) &-&-&-&- &- \\
\hline
$N_{QUB1}^{CIC}$ & $N_{QUB1}^{UNSW}$   & CW (\textit{default parameter}) &-&-&-&- &- \\

\hline
\(N_{QUB2}^{UNSW}\) & \(N_{QUB2}^{CIC}\)  & I-FGSM (\epsilon=0.1) & 35.58 & 2.91 & 10.07 & 1.00 & 0.98\\
\hline
\(N_{QUB2}^{UNSW}\) & \(N_{QUB2}^{CIC}\)   & I-FGSM (\epsilon=0.01) & 35.94 &2.79 & 9.64 & 1.00 & 0.98\\ 
\hline
\(N_{QUB2}^{UNSW}\) & \(N_{QUB2}^{CIC}\)   & I-FGSM (\epsilon=0.001) &36.00&2.77 &9.53 &1.00 &1.00 \\
\hline
\(N_{QUB2}^{UNSW}\) & \(N_{QUB2}^{CIC}\)  & FGSM (\epsilon=0.1) &25.79 &10.12 &17.74 &1.00 &1.00 \\
\hline
\(N_{QUB2}^{UNSW}\) & \(N_{QUB2}^{CIC}\)   & FGSM (\epsilon=0.01) &25.87 &10.04 &17.59 &1.00 &1.00 \\
\hline
\(N_{QUB2}^{UNSW}\) & \(N_{QUB2}^{CIC}\)  & FGSM (\epsilon=0.001) &25.97 &9.92 &17.36 &1.00 &1.00 \\
\hline
\(N_{QUB2}^{UNSW}\) & \(N_{QUB2}^{CIC}\)  & JSMA (\theta=0.1) &32.41 &0.36 &178.50 &1.00 &0.03 \\
\hline
\(N_{QUB2}^{UNSW}\) & \(N_{QUB2}^{CIC}\)   & JSMA (\theta=0.01) &-&-&-&- &FAIL \\
\hline
\(N_{QUB2}^{UNSW}\) & \(N_{QUB2}^{CIC}\)   & LBFGS (\textit{default parameter})&24.90& 7.20 & 135.18 &1.00&0.81 \\
\hline
\(N_{QUB2}^{UNSW}\) & \(N_{QUB2}^{CIC}\)  & PGD (\textit{default parameter})&35.79 &2.87 &9.27 &1.00 &0.91 \\
\hline
\(N_{QUB2}^{UNSW}\) & \(N_{QUB2}^{CIC}\) & DeepFool (\textit{default parameter}) &-&-&-&- &- \\
\hline
\(N_{QUB2}^{UNSW}\) & \(N_{QUB2}^{CIC}\)  & CW (C=100) &40.19&0.90&31.59&1.00 &0.63 \\
\hline

 \(N_{QUB2}^{CIC}\) & \(N_{QUB2}^{UNSW}\)  & I-FGSM (\epsilon=0.1) & 40.38 & 1.81 & 4.32 & 1.00 & 0.54\\
\hline
\(N_{QUB2}^{CIC}\) & \(N_{QUB2}^{UNSW}\)  & I-FGSM (\epsilon=0.01) & 40.05 &1.89 & 4.51 & 1.00 & 0.47\\ 
\hline
\(N_{QUB2}^{CIC}\) & \(N_{QUB2}^{UNSW}\)   & I-FGSM (\epsilon=0.001) &40.02 &1.90 &4.52 &1.00 &0.47 \\
\hline
\(N_{QUB2}^{CIC}\) & \(N_{QUB2}^{UNSW}\)  & FGSM (\epsilon=0.1) &44.70 &1.32 &1.90 &1.00 &0.86 \\
\hline
\(N_{QUB2}^{CIC}\) & \(N_{QUB2}^{UNSW}\)  & FGSM (\epsilon=0.01) &41.62 &1.76 &2.57 &1.00 &0.85 \\
\hline
\(N_{QUB2}^{CIC}\) & \(N_{QUB2}^{UNSW}\)  & FGSM (\epsilon=0.001) &45.53 &0.20 &1.71 &1.00 &0.85 \\
\hline
\(N_{QUB2}^{CIC}\) & \(N_{QUB2}^{UNSW}\) & JSMA (\theta=0.1) &42.93 &0.23 &41.87 &1.00 &0.99 \\
\hline
\(N_{QUB2}^{CIC}\) & \(N_{QUB2}^{UNSW}\)  & JSMA (\theta=0.01) &42.86 &0.27 &44.55 &1.00 &0.88 \\
\hline
\(N_{QUB2}^{CIC}\) & \(N_{QUB2}^{UNSW}\)  & LBFGS (\textit{default parameter})&-&-&-&-&- \\
\hline
\(N_{QUB2}^{CIC}\) & \(N_{QUB2}^{UNSW}\)  & PGD (\textit{default parameter})&41.27 &1.69 &3.45 &1.00 &0.44 \\
\hline
\(N_{QUB2}^{CIC}\) & \(N_{QUB2}^{UNSW}\)  & DeepFool (\textit{default parameter}) &-&-&-&- &- \\
\hline
\(N_{QUB2}^{CIC}\) & \(N_{QUB2}^{UNSW}\)   & CW (\textit{default parameter}) &-&-&-&- &- \\
\hline
\end{tabular}
}
\caption{Cross Training 1 & 2}
\end{table}

==> Tables/DefenseMPA.tex <==
\begin{table*}[!h]
%\scriptsize
\centering
\caption{\violet{Test Accuracy Values TN with an MPA fine-tunning.} \label{Defense_MPA}}
\begin{tabular}{@{}|>{\color{violet}}c |>{\color{violet}}c |>{\color{violet}}c |>{\color{violet}}c |>{\color{violet}}c |>{\color{violet}}c | >{\color{violet}}c |}
\hline
\textbf{TN} & \textbf{Fine-Tune} & \textbf{Parameter} & \textbf{I-FGSM, $\varepsilon$ = 0.01} & \textbf{IFGSM, $\varepsilon$ = 0.001} &\textbf{LBFGS, Default} &\textbf{JSMA, $\theta$ = 0.01}\TBstrut\\
 \hline
 \rowcolor{grey}
 
$N_{SPRITZ1}^{N-BaIoT}$ & JSMA & $\theta$ = 0.01 & 0.0000 & 0.0100 & 0.2010 & ---\TBstrut\\ \hline

$N_{SPRITZ1}^{DGA}$ & I-FGSM& $\varepsilon$ = 0.01 & --- & 0.0000 & 0.0010 & 0.0000\TBstrut\\ \hline
 \rowcolor{grey}

$N_{SPRITZ1}^{DGA}$ & I-FGSM& $\varepsilon$ = 0.001 & 0.0000 & --- & 0.0010 & 0.0000\TBstrut\\ \hline

$N_{SPRITZ1}^{DGA}$ & LBFGS& Default & 0.0200 & 0.0010 & --- & 0.0000\TBstrut\\ \hline

%SPRITZ1 & I-FGSM, $\varepsilon$ = 0.01 & N-BaIoT & DGA& 20.49 &21.57\TBstrut\\ %\hline
 %\rowcolor{grey}
%SPRITZ1 & I-FGSM, $\varepsilon$ = 0.001 & N-BaIoT &DGA& 203.98 & 212.77\TBstrut\\ %\hline

%SPRITZ1 & JSMA, $\theta$ = 0.1 & N-BaIoT &DGA& 30.41 & 10.42\TBstrut\\ \hline
 %\rowcolor{grey}
%SPRITZ1 & LBFGS, default parameter & N-BaIoT &DGA& 48.73 & 25.92\TBstrut\\ \hline

%SPRITZ1 & PGD, default parameter & N-BaIoT &DGA& 16.92 & 16.17\TBstrut\\ \hline
 %\rowcolor{grey}
%SPRITZ1 & DeepFool, default parameter & N-BaIoT &DGA& 0.49 &0.23\TBstrut\\ \hline
%

%SPRITZ2 & I-FGSM, $\varepsilon$ = 0.1 & N-BaIoT & DGA& 4.42& 4.49\TBstrut\\ \hline
%\rowcolor{grey}
%SPRITZ2 & I-FGSM, $\varepsilon$ = 0.01 & N-BaIoT & DGA& 43.94 &44.98\TBstrut\\ %\hline
 
%SPRITZ2 & I-FGSM, $\varepsilon$ = 0.001 & N-BaIoT &DGA& 438.436 & 446.969\TBstrut\\ \hline
%\rowcolor{grey}
%SPRITZ2 & JSMA, $\theta$ = 0.1 & N-BaIoT &DGA& 32.58 & 20.53\TBstrut\\ \hline
 
%SPRITZ2 & LBFGS, default parameter & N-BaIoT &DGA& 78.73 & 51.93\TBstrut\\ \hline
%\rowcolor{grey}
%SPRITZ2 & PGD, default parameter & N-BaIoT &DGA& 45.25 & 33.60\TBstrut\\ \hline
 
%SPRITZ2 & DeepFool, default parameter & N-BaIoT &DGA& 0.31 &0.37\TBstrut\\ \hline 
%$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{N-BaIoT}$ & SN = 98.90\% , TN = 98.80\% & JSMA, $\theta$ = 0.1 & 18.49 & 7.29 & 170.50 & 1.0000 & 1.0000 \TBstrut\\ \hline

%$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{DGA}$ & SN = 99.60\% , TN = 99.60\% & I-FGSM, $\varepsilon$ = 0.01 & 28.62 & 5.99 & 23.25 & 1.0000 & 1.0000 \TBstrut\\ \hline
% \rowcolor{grey}
%$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{DGA}$ & SN = 99.60\% , TN = 99.60\% & I-FGSM, $\varepsilon$ = 0.001 & 28.92 & 5.76 & 22.64 & 1.0000 & 1.0000 \TBstrut\\ \hline

%$N_{SPRITZ2}^{N-BaIoT}$ & $N_{SPRITZ1}^{N-BaIoT}$ & SN = 98.90\% , TN = 98.80\% & JSMA, $\theta$ = 0.01 & 40.93 & 0.30 & 17.84 & 1.0000 & 0.9960 \TBstrut\\ \hline
 %\rowcolor{grey}
%$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{DGA}$ & SN = 99.60\% , TN = 99.60\% & LBFGS, default parameter &  34.22 & 1.48 & 33.92 & 0.9930 & 0.6300 \TBstrut\\ \hline

\end{tabular}
\end{table*}


==> Tables/Differences.tex <==
\begin{table*}[!h]
\centering
%\scriptsize
\caption{Differences between our study and existing studies} \label{difference}
%\begin{tabular}{|l|l|l|l|l|l|}
\resizebox{2\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Ref.} & \textbf{App. Domain} & \textbf{Adv. Attacks} & \textbf{Datasets} & \textbf{Results}   \\ \hline

%\cite{Barni2019OnForensics} & Image forensics & -JSMA, I-FGSM             &      -RAISE~\cite{dang2015raise}, and VISION~\cite{shullani2017vision}                  & -Non transferable                        \\ \hline

 \cite{Marra2018OnIdentification}    &    Image forensics                &   -FGSM, PGD     &            -VISION~\cite{shullani2017vision} & -Non transferable\\\hline
   
\cite{WangAdmix:Attacks}      &   Computer vision   &     -Inp. transformation         &     -ImageNet~\cite{russakovsky2015imagenet} & -Few cases transfer, but Fails in other domains\\\hline

   
\cite{Jia2019EnhancingReduction}     &   Computer vision                 &       -Dispersion reduction    &            -ImageNet~\cite{russakovsky2015imagenet}   &   -Enhancing distortion degrades model performance\\ \hline

 \cite{SuciuWhenAttacksb} &   Various domains &     StingRay      &    -Drebin~\cite{arp2014drebin}      &   - Fails in small perturbations in the examples.  \\\hline
 

\cite{DemontisWhyAttacks}        & Various domains   &        -Gradient attack            &    -MNIST89~\cite{deng2012mnist}, and Drebin~\cite{arp2014drebin} &  - Fails in multi-class classification   \\\hline

\cite{Nowroozi2022Dem}        & Computer networks   &        -JSMA and I-FGSM      &  N-BaIoT\cite{Abbasi2021}, RIPE\cite{staff2015ripe}, and DGA\cite{upadhyay2020}   &  - Non Transferable \\\hline

\multirow{2}{*}{Our's} & \multirow{2}{*}{Computer Networks} & \multirow{2}{*}{\begin{tabular}{@{}c@{}}-FGSM, I-FGSM, JSMA, PGD,\\ L-BFGS, CW\end{tabular}} & \multirow{2}{*}{UNSW\cite{UNSW-Dataset}, and CIC\cite{CIC-Dataset}} & \multirow{2}{*}{- Complete Transferable between SN and TN} \\
 & & & & \\
\hline

\end{tabular}}
\end{table*}

==> Tables/Transferability.tex <==
\begin{table*}[!h]
%\scriptsize
\centering
\caption{Summary of Transferability cases. \label{Transferability}}
\begin{tabular}{@{}|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{SN} & \textbf{TN} & \textbf{Accuracy} & \textbf{Attack Type} & \textbf{PSNR} & \textbf{$L_1$ dist} & \textbf{Max. dist} & \textbf{ASR} & \textbf{ASR} \TBstrut\\
& & & & & & & \textbf{(SN)} & \textbf{(TN)}  \\ \hline
 \rowcolor{grey}
$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{N-BaIoT}$ & SN = 98.90\% , TN = 98.80\% & JSMA, $\theta$ = 0.1 & 18.49 & 7.29 & 170.50 & 1.0000 & 1.0000 \TBstrut\\ \hline

$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{DGA}$ & SN = 99.60\% , TN = 99.60\% & I-FGSM, $\varepsilon$ = 0.01 & 28.62 & 5.99 & 23.25 & 1.0000 & 1.0000 \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{DGA}$ & SN = 99.60\% , TN = 99.60\% & I-FGSM, $\varepsilon$ = 0.001 & 28.92 & 5.76 & 22.64 & 1.0000 & 1.0000 \TBstrut\\ \hline

$N_{SPRITZ2}^{N-BaIoT}$ & $N_{SPRITZ1}^{N-BaIoT}$ & SN = 98.90\% , TN = 98.80\% & JSMA, $\theta$ = 0.01 & 40.93 & 0.30 & 17.84 & 1.0000 & 0.9960 \TBstrut\\ \hline
 \rowcolor{grey}
$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{DGA}$ & SN = 99.60\% , TN = 99.60\% & LBFGS, default parameter &  34.22 & 1.48 & 33.92 & 0.9930 & 0.6300 \TBstrut\\ \hline

\end{tabular}
\end{table*}

==> Tables/executionTime.tex <==
\begin{table*}[!th]
%\scriptsize
\centering
\caption{\red{Execution running attack time on SN.} \label{Exe_Time}}
\resizebox{2\columnwidth}{!}{
\begin{tabular}{@{}|>{\color{red}}c |>{\color{red}}c |>{\color{red}}c |>{\color{red}}c |>{\color{red}}c |>{\color{red}}c |>{\color{red}}c |>{\color{red}}c|}
\hline
\textbf{SN} & \textbf{Attack Type} & \textbf{Dataset1} & \textbf{Dataset2} & \textbf{Dataset3}& \textbf{Exe. min (Dataset1)} &\textbf{Exe. min (Dataset2)} &\textbf{Exe. min (Dataset3)}\TBstrut\\
 \hline
 \rowcolor{grey}
 
SPRITZ1 & I-FGSM, $\varepsilon$ = 0.1 & N-BaIoT & DGA&RIPE &2.12& 2.13&2.18\TBstrut\\ \hline

SPRITZ1 & I-FGSM, $\varepsilon$ = 0.01 & N-BaIoT & DGA&RIPE & 20.49 &21.57& ---\TBstrut\\ \hline
 \rowcolor{grey}
SPRITZ1 & I-FGSM, $\varepsilon$ = 0.001 & N-BaIoT &DGA&RIPE & 203.98 & 212.77& ---\TBstrut\\ \hline

SPRITZ1 & JSMA, $\theta$ = 0.1 & N-BaIoT &DGA&RIPE & 30.41 & 10.42&30.67\TBstrut\\ \hline
 \rowcolor{grey}
SPRITZ1 & LBFGS, default parameter & N-BaIoT &DGA&RIPE & 48.73 & 25.92& 40.92\TBstrut\\ \hline

SPRITZ1 & PGD, default parameter & N-BaIoT &DGA&RIPE & 16.92 & 16.17, &16.27\TBstrut\\ \hline
 \rowcolor{grey}
SPRITZ1 & DeepFool, default parameter & N-BaIoT &DGA&RIPE &0.49 &0.23&0.38\TBstrut\\ \hline
%

SPRITZ2 & I-FGSM, $\varepsilon$ = 0.1 & N-BaIoT & DGA& RIPE &4.42& 4.49& ---\TBstrut\\ \hline
\rowcolor{grey}
SPRITZ2 & I-FGSM, $\varepsilon$ = 0.01 & N-BaIoT & DGA&RIPE & 43.94 &44.98& ---\TBstrut\\ \hline
 
SPRITZ2 & I-FGSM, $\varepsilon$ = 0.001 & N-BaIoT &DGA&RIPE & 438.436 & 446.969& ---\TBstrut\\ \hline
\rowcolor{grey}
SPRITZ2 & JSMA, $\theta$ = 0.1 & N-BaIoT &DGA&RIPE & 32.58 & 20.53& ---\TBstrut\\ \hline
 
SPRITZ2 & LBFGS, default parameter & N-BaIoT &DGA&RIPE & 78.73 & 51.93& ---\TBstrut\\ \hline
\rowcolor{grey}
SPRITZ2 & PGD, default parameter & N-BaIoT &DGA&RIPE & 45.25 & 33.60& ---\TBstrut\\ \hline
 
SPRITZ2 & DeepFool, default parameter & N-BaIoT &DGA&RIPE & 0.31 &0.37 & ---\TBstrut\\ \hline 
%$N_{SPRITZ1}^{N-BaIoT}$ & $N_{SPRITZ2}^{N-BaIoT}$ & SN = 98.90\% , TN = 98.80\% & JSMA, $\theta$ = 0.1 & 18.49 & 7.29 & 170.50 & 1.0000 & 1.0000 \TBstrut\\ \hline

%$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{DGA}$ & SN = 99.60\% , TN = 99.60\% & I-FGSM, $\varepsilon$ = 0.01 & 28.62 & 5.99 & 23.25 & 1.0000 & 1.0000 \TBstrut\\ \hline
% \rowcolor{grey}
%$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{DGA}$ & SN = 99.60\% , TN = 99.60\% & I-FGSM, $\varepsilon$ = 0.001 & 28.92 & 5.76 & 22.64 & 1.0000 & 1.0000 \TBstrut\\ \hline

%$N_{SPRITZ2}^{N-BaIoT}$ & $N_{SPRITZ1}^{N-BaIoT}$ & SN = 98.90\% , TN = 98.80\% & JSMA, $\theta$ = 0.01 & 40.93 & 0.30 & 17.84 & 1.0000 & 0.9960 \TBstrut\\ \hline
 %\rowcolor{grey}
%$N_{SPRITZ2}^{DGA}$ & $N_{SPRITZ1}^{DGA}$ & SN = 99.60\% , TN = 99.60\% & LBFGS, default parameter &  34.22 & 1.48 & 33.92 & 0.9930 & 0.6300 \TBstrut\\ \hline

\end{tabular}}
\end{table*}


==> Transactions-Bibliography/README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

IEEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************

